Runtime Enforcement of CPS against Signal Temporal Logic

Cyber-Physical Systems (CPSs), especially those involving autonomy, need guarantees of their safety. Runtime Enforcement (RE) is a lightweight method to formally ensure that some specified properties are satisfied over the executions of the system. Hence, there is recent interest in the RE of CPS. However, existing methods are not designed to tackle specifications suitable for the hybrid dynamics of CPS. With this in mind, we develop runtime enforcement of CPS using properties defined in Signal Temporal Logic (STL). In this work, we aim to construct a runtime enforcer for a given STL formula to minimally modify a signal to satisfy the formula. To achieve this, the STL formula to be enforced is first translated into a timed transducer, while the signal to be corrected is encoded as timed words. We provide timed transducers for the temporal operators \emph{until} and \emph{release} noting that other temporal operators can be expressed using these two. Our approach enables effective enforcement of STL properties for CPS. A case study is provided to illustrate the approach and generate empirical evidence of its suitability for CPS.

==> macros.tex <==
% !TEX root = ./main.tex
%
\RequirePackage{todonotes}

% TODOS
%\setlength{\marginparwidth}{1.5cm}

\newcommand{\saucomment}[1]{\todo[color=Violet!25,size=\small,fancyline,author=Saumya]{#1}\xspace}
\newcommand{\saucommentinline}[1]{\todo[inline,color=Violet!25,author=Saumya]{#1}\xspace}
\newcommand{\atsau}{\colorbox{Violet!25}{\textbf{@Saumya}}}

\newcommand{\hscomment}[1]{\todo[color=cyan!30,size=\small,fancyline,author=Han]{#1}\xspace}
\newcommand{\hscommentinline}[1]{\todo[inline,color=cyan!30,author=Han]{#1}\xspace}
\newcommand{\aths}{\colorbox{cyan!30}{\textbf{@Han}}}

\newcommand{\prcomment}[1]{\todo[color=orange!25,size=\small,fancyline,author=Partha]{#1}\xspace}
\newcommand{\prcommentinline}[1]{\todo[inline,color=orange!25,author=Partha]{#1}\xspace}
\newcommand{\atpr}{\colorbox{orange!25}{\textbf{@Partha}}}

\newcommand{\nzcomment}[1]{\todo[color=blue!25,size=\small,fancyline,author=Naijun]{#1}\xspace}
\newcommand{\nzcommentinline}[1]{\todo[inline,color=blue!25,author=Naijun]{#1}\xspace}
\newcommand{\atnz}{\colorbox{blue!25}{\textbf{@Naijun}}}

\newcommand{\spcomment}[1]{\todo[color=ForestGreen!25,size=\small,fancyline,author=Srinivas]{#1}\xspace}
\newcommand{\spcommentinline}[1]{\todo[inline,color=ForestGreen!25,author=Srinivas]{#1}\xspace}
\newcommand{\atsp}{\colorbox{ForestGreen!25}{\textbf{@Srinivas}}}

%colors
\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\nblue}[1]{\textcolor{NavyBlue}{#1}}
\newcommand{\red}[1]{\textcolor{Red}{#1}}
\newcommand{\orange}[1]{\textcolor{RedOrange}{#1}}
\newcommand{\gray}[1]{\textcolor{Gray}{#1}}
\newcommand{\maroon}[1]{\textcolor{Maroon}{#1}}
\newcommand{\violet}[1]{\textcolor{Violet}{#1}}
\newcommand{\black}[1]{\textcolor{Black}{#1}} 

\newcommand{\customcite}[2]{[\citealp{#1}, #2]}

% Real, Natural ...
\newcommand{\Reals}{\mathbb{R}\xspace}
\newcommand{\PosReals}{\mathbb{R}_{> 0}\xspace}
\newcommand{\NonNegReals}{\mathbb{R}_{\ge 0}\xspace}
\newcommand{\Realn}{\mathbb{R}^n\xspace}
\newcommand{\Nats}{\mathbb{N}\xspace}
\newcommand{\PosNats}{\mathbb{N}_{>0}\xspace}
\newcommand{\Ints}{\mathbb{Z}\xspace}
\newcommand{\Boolean}{\mathbb{B}\xspace}
\newcommand{\NonNegRat}{\mathbb{Q}_{\ge 0}\xspace}
%% Symbol
\newcommand{\Def}{\mathrel{::=}}
\newcommand{\power}[1]{\ensuremath{2^{#1}}\xspace}

%% STL Tempotal Operators
\newcommand{\until}[1][]{\ensuremath{\mathcal{U}\ifthenelse{\equal{#1}{}}{}{\ifthenelse{\pdfmatch{,}{#1}=1}{_{[#1]}}{_{#1}}}}\xspace}
\newcommand{\release}[1][]{\ensuremath{\mathcal{R}\ifthenelse{\equal{#1}{}}{}{\ifthenelse{\pdfmatch{,}{#1}=1}{_{[#1]}}{_{#1}}}}\xspace}
\newcommand{\always}[1][]{\ensuremath{\Box\ifthenelse{\equal{#1}{}}{}{\ifthenelse{\pdfmatch{,}{#1}=1}{_{[#1]}}{_{#1}}}}\xspace}
\newcommand{\eventually}[1][]{\ensuremath{\Diamond\ifthenelse{\equal{#1}{}}{}{\ifthenelse{\pdfmatch{,}{#1}=1}{_{[#1]}}{_{#1}}}}\xspace}
\newcommand{\signal}{\bm{x}\xspace}
% \llangle for [[, \rragnel for ]]
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1[}\)}%
  \mathopen{\copy\@brx\kern-0.6\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1]}\)}%
  \mathclose{\copy\@brx\kern-0.6\wd\@brx\usebox{\@brx}}}
\makeatother



%% Timed Automata Syntax
\newcommand{\tword}{\bm{\sigma}\xspace}
\newcommand{\emptyword}{\bm{\epsilon}\xspace}
\newcommand{\resltsig}{\bm{o}\xspace}
\newcommand{\clock}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\clockreset}[2][v]{\ensuremath{{#1}[#2\!\leftarrow\!0]}\xspace}
\newcommand{\automaton}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\alphbt}{\ensuremath{\Sigma}\xspace}
\newcommand{\ap}{\ensuremath{\mathtt{AP}}\xspace}
\newcommand{\loca}{\ensuremath{L}\xspace}
\newcommand{\linit}{\ensuremath{l_0}\xspace}
\newcommand{\lacpt}{\ensuremath{F}\xspace}
\newcommand{\trans}{\ensuremath{\Delta}\xspace}


%%%%    Shortcuts    %%%%
\newcommand{\tiff}{\textnormal{iff}\quad}
\newcommand{\qiff}{\ \quad\textnormal{iff}\quad\ }
\newcommand{\qqiff}{\qquad\textnormal{iff}\qquad}
\newcommand{\lqiff}{\textnormal{iff}\quad}
\newcommand{\lqqiff}{\textnormal{iff}\qquad}

\newcommand{\aand}{\ \ \textnormal{and}\ \ }
\newcommand{\qand}{\ \quad\textnormal{and}\quad\ }
\newcommand{\qqand}{\qquad\textnormal{and}\qquad}
\newcommand{\oor}{\ \ \textnormal{or}\ \ }
\newcommand{\qor}{\ \quad\textnormal{or}\quad\ }
\newcommand{\qqor}{\qquad\textnormal{or}\qquad}

\newcommand{\suchthat}{\textnormal{such that}\ \ }
\newcommand{\qsuchthat}{\ \quad\textnormal{such that}\quad\ }
\newcommand{\qqsuchthat}{\qquad\textnormal{such that}\qquad}


\makeatletter
\newcommand*{\Frac}[2]{%
  % Even numbered box and register numbers smaller than 10 are
  % for local assignments.
  \begingroup
    % "Numerator" in box 0
    \sbox0{$#1\m@th$}%
    % "Denominator" in box 2
    \sbox2{$#2\m@th$}%
    % Maximum width in \dimen2
    \ifdim\wd0 > \wd2 %
      \dimen0=\wd0 %
    \else
      \dimen0=\wd2 %
    \fi
    % Add overshoot (5pt) of the line
    \advance\dimen0 by 10pt\relax
    % Vertical separation
    \dimen2=3pt\relax
    \setbox4=\vbox{%
      \hbox to \dimen0{\hfill\unhcopy0\hfill}%
      \kern\dimen2
      \hrule % default line thickness: 0.4pt
      \kern\dimen2
      \hbox to \dimen0{\hfill\unhcopy2\hfill}%
      \kern0pt\relax
    }%
    % Box for measuring height of math axis
    \sbox0{$\vcenter{}$}%
    % Set result with the line at the math axis
    \raise\dimexpr\ht0 - \ht2 - \dp2 - \dimen2 - .2pt\relax\copy4 %
  \endgroup
}
\makeatother
\newcommand{\TAG}[1]{{\tag*{\small{[{#1}]}}}}

\DeclareMathOperator*{\argmin}{arg\,min} 
\DeclareMathOperator*{\argmax}{arg\,max}
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother

==> sections/Propositions1.tex <==
NOT CORRECT
\color{red}
    Proposition 1: Given an STL formula $p_1\until_{[a,b]}p_2$ and given $\signal$ be the signals to be corrected, then output of the enforcer $E_{p_1\until_{[a,b]}p_2}$ satisfies $p_1\until_{[a,b]}p_2$, i.e., 
        \begin{align*}
            E_{p_1\until_{[a,b]}p_2}(\signal, t) \models p_1\until_{[a,b]}p_2
        \end{align*}

  
Let us consider the following cases based on time intervals: $[0, a), [a,b), b$.
\begin{enumerate}
        \item [Case 1:] For signals $\signal$ received between $[0, a)$.\\
        \begin{enumerate}
            \item [Case a:] Consider the encoded input event is $p_1$ for $\signal$:\\
            
            According to the semantics of STL from Definition \ref{def:STL Semantics} $p_1$ should be continuously true at all times $t \in [0, a)$. This case considers $p_1$ being received at $t \in [0, a)$, so STL formula is satisfied by the signal values (consequently, signal should be released without modification). Thus, 
            \begin{align}
            \label{1}
                \signal \models p_1\until_{[a,b]}p_2
            \end{align}

            Now, for $p_1$, $\automaton_{p_1\until_{[a,b]}p_2}$ in Figure \ref{fig: until} for $t \in [0, a)$ outputs $\top$, and the enforcer $E_{p_1\until_{[a,b]}p_2}$ for $output=\top$ just releases the signal without modification. Thus,
            \begin{align}
            \label{2}
                E_{p_1\until_{[a,b]}p_2}(\signal, t)=\signal
            \end{align}

            From Equations \ref{1} and \ref{2},  $E_{p_1\until_{[a,b]}p_2}(\signal, t) \models p_1\until_{[a,b]}p_2$. \\~\\

            
            \item [Case b:] For $\signal$, consider the encoded input event is $\neg p_1$:\\
            
            According to the semantics of STL from Definition \ref{def:STL Semantics} $p_1$ should be continuously true at all times $t \in [0, a)$. This case considers $\neg p_1$ being received at $t \in [0, a)$. So, the STL formula is not satisfied by the signal values. \\%(consequently, signal $\signal$ should be corrected to $\signal'$ to satisfy proposition $p_1$ and then released). Thus, 
            
            $\automaton_{p_1\until_{[a,b]}p_2}$ considering $p_1$ and  $t \in [0, a)$, outputs $\bot_1$, and the enforcer $E_{p_1\until_{[a,b]}p_2}$ reconstructs and outputs the signal $\signal'$, i.e.,
            \begin{equation}    
            \begin{split}
            \label{3}
                \signal \not \models p_1\until_{[a,b]}p_2 \implies \exists\signal', E_{p_1\until_{[a,b]}p_2}(\signal, t)=\signal' : \\(min(|\signal'-\signal|) \land p_1(\signal')=\top \land (\signal'\models p_1\until_{[a,b]}p_2))
            \end{split}
            \end{equation}    

            From Equations \ref{3},  $E_{p_1\until_{[a,b]}p_2}(\signal, t) \models p_1\until_{[a,b]}p_2$. \\~\\
        \end{enumerate}
        
        \item [Case 2:] For signals $\signal$ received between $[a,b)$.\\
            \begin{enumerate}
                \item [Case a:] For $\signal$, consider the encoded input event is $p_2 \land p_1$:\\
                
                According to the semantics of STL from Definition \ref{def:STL Semantics}, if  $p_2$ is true at  $t \in [a, b)$, the STL formula is satisfied by the signal values given $p_1$ is also true, i.e., 
                \begin{align}
                    \label{4}
                        \signal \models p_1\until_{[a,b]}p_2
                \end{align}
                Now, for $p_2 \land p_1$, $\automaton_{p_1\until_{[a,b]}p_2}$ in Figure \ref{fig: until} for $t \in [a, b)$ outputs $\top$, and the enforcer $E_{p_1\until_{[a,b]}p_2}$ for $output=\top$ just releases the signal without modification. Thus,
                \begin{align}
                \label{5}
                    E_{p_1\until_{[a,b]}p_2}(\signal, t)=\signal
                \end{align}
                From Equations \ref{4} and \ref{5},  $E_{p_1\until_{[a,b]}p_2}(\signal, t) \models p_1\until_{[a,b]}p_2$. \\~\\
                
                \item [Case b:] For $\signal$, consider the encoded input event is $p_2 \land \neg p_1$:\\
                
                According to the semantics of STL from Definition \ref{def:STL Semantics}, if  $p_2$ is true at  $t \in [a, b)$, the STL formula is satisfied by the signal values, given $p_1$ is also true. However, this case considers $\neg p_1$ being received at $t \in [a, b)$. So, the STL formula is not satisfied by the signal values.\\
                
                $\automaton_{p_1\until_{[a,b]}p_2}$ considering $p_2 \land \neg p_1$ and  $t \in [a,b) $, outputs $\bot_1$, and the enforcer $E_{p_1\until_{[a,b]}p_2}$ reconstructs and outputs the signal $\signal'$, i.e.,
            \begin{equation}    
            \begin{split}
            \label{6}
                \signal \not \models p_1\until_{[a,b]}p_2 \implies \exists\signal', E_{p_1\until_{[a,b]}p_2}(\signal, t)=\signal' : \\(min(|\signal'-\signal|) \land p_1(\signal')=\top \land p_2(\signal')=\top \land (\signal'\models p_1\until_{[a,b]}p_2))
            \end{split}
            \end{equation}  
            From Equations \ref{6},  $E_{p_1\until_{[a,b]}p_2}(\signal, t) \models p_1\until_{[a,b]}p_2$. \\~\\
            
                \item [Case c:] For $\signal$, consider the encoded input event is $\neg p_2 \land p_1$:\\
                    
                As per the semantics of $\varphi_1\until_{[a,b]}\varphi_2$ of STL, $p_1$ should be continuously true for $t \in [a,b) $ which is considered in this case.\\

                $\automaton_{p_1\until_{[a,b]}p_2}$ considering $\neg p_2 \land p_1$ and  $t \in [a,b) $, outputs $\top$, and the enforcer $E_{p_1\until_{[a,b]}p_2}$ for $output=\top$ just releases the signal without modification. Thus,
                \begin{align}
                \label{5}
                    E_{p_1\until_{[a,b]}p_2}(\signal, t)=\signal
                \end{align}
                From Equations \ref{4} and \ref{5},  $E_{p_1\until_{[a,b]}p_2}(\signal, t) \models p_1\until_{[a,b]}p_2$. \\~\\
        
                \item [Case d:] For $\signal$, consider the encoded input event is $\neg p_2 \land \neg p_1$:\\
                As per the semantics of $\varphi_1\until_{[a,b]}\varphi_2$ of STL, $p_1$ should be continuously true for $t \in [a,b) $. However, this case considers $\neg p_1$ being received at $t \in [a, b)$. So, the STL formula is not satisfied by the signal values.\\
                
                $\automaton_{p_1\until_{[a,b]}p_2}$ considering $\neg p_2 \land \neg p_1$ and  $t \in [a,b) $, outputs $\bot_1$, and the enforcer $E_{p_1\until_{[a,b]}p_2}$ reconstructs and outputs the signal $\signal'$, i.e.,
            \begin{equation}    
            \begin{split}
            \label{6}
                \signal \not \models p_1\until_{[a,b]}p_2 \implies \exists\signal', E_{p_1\until_{[a,b]}p_2}(\signal, t)=\signal' : \\(min(|\signal'-\signal|) \land p_1(\signal')=\top  \land (\signal'\models p_1\until_{[a,b]}p_2))
            \end{split}
            \end{equation}  
            From Equations \ref{6},  $E_{p_1\until_{[a,b]}p_2}(\signal, t) \models p_1\until_{[a,b]}p_2$. \\~\\
            
            \end{enumerate}
        

        
        \item [Case 3:] For signals $\signal$ received at $b$.\\
    \end{enumerate}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Proposition 2: Given an STL formula $p_1\release_{[a,b]}p_2$ and given $\signal$ be the signals to be corrected, then output of the enforcer $E_{p_1\release_{[a,b]}p_2}$ satisfies $p_1\release_{[a,b]}p_2$, i.e., 
        \begin{align*}
            E_{p_1\release_{[a,b]}p_2}(\signal, t) \models p_1\release_{[a,b]}p_2
        \end{align*}

==> sections/operators/eventually.tex <==
\subsubsection{Timed Automaton for $\eventually_{[0,a]}\varphi$}
        We let $\automaton=(\loca,\linit,\clock,\allowbreak\alphbt,\trans, Inv, \lambda, \lacpt)$, where
        \begin{itemize}
            \item $\loca=\{l_0, l_1, l_2, l_3\}$ where $observing=\{l_0, l_1\}$, $modifying=\{l2\}$ and $violation=\{l3\}$
            \item $\linit=l_0$ 
            \item $\clock=\{c\}$
            \item $\allowbreak\alphbt=\{\varphi, \neg \varphi\}$
            \item $\trans=\{ \delta_1, \delta_2, \delta_3,\delta_4, \delta_5, \delta_6, \delta_7, \delta_8,\delta_9 \}$
            \item \sout{$Inv(l_2): x<a$} \\
            $Inv=\{(l_0,\emptyset),(l_1,\emptyset), (l_2, c<a)\}$
            \item $\lambda=\{\lambda_1, \lambda_2, \lambda_3, \lambda_4, \lambda_5, \lambda_6, \lambda_7, \lambda_8, \lambda_9\}$
            \item \sout{$\lacpt=\{l_1\}$}
        \end{itemize}

        \begin{table}[H]
        \begin{tabular}{@{}ccc@{}}
        \hline
        i & $\delta_i$                   & $\lambda_i$ \\ \hline
        1 & $(l_0, \varphi, \epsilon, \epsilon, l_2)$ & $\mu(x)$  \\ 
        2 & $(l_0, \neg \varphi, \epsilon, c:=0, l_1)$ & $\mu(x)$  \\ 
        3 & $(l_1, \varphi, \epsilon, \epsilon, l_1)$ & $\mu(x)$  \\ 
        4 & $(l_1, \neg \varphi, \epsilon, c:=0, l_2)$ & $\mu(x)$  \\ 
        5 & $(l_2, \neg \varphi, c==a, c:=0, l_2)$ & $\mu(x)=0.7$  \\ 
        6 & $(l_2, \varphi, c \leq a, \epsilon, l_1)$ & $\mu(x)$  \\ 
        7 & $(l_2, \neg \varphi, c<a, \epsilon, l_2)$ & $\mu(x)$  \\ 
        8 & $(l_2, \top, c>a, \epsilon, l_3)$ & $vio$  \\ 
        9 & $(l_3, \top, \epsilon, \epsilon, l_1)$ & $vio$  \\ \bottomrule
        \end{tabular}
        \caption
        {Edges of TA of $\eventually_{[0,c]}\varphi$ and their output labels.}
        \end{table}


        \begin{figure}[H]
            \centering
            \begin{tikzpicture}[->,shorten >=1pt,auto,node distance=3.5cm,el/.style = {inner sep=2pt, align=left, sloped},every label/.append style = {font=\small},semithick,initial where=above]
			
			\tikzstyle{every node}=[font=\small]
			\tikzstyle{good state}=[circle,thick,draw=blue!75,fill=blue!20,minimum size=5mm,accepting]
			\tikzstyle{bad state}=[circle,thick,draw=red!75,fill=red!20,minimum size=3mm]
			\tikzstyle{dead state}=[rectangle,thick,draw=red!75,fill=red!20,minimum size=5mm]

            \node[initial,bad state] (S0) {$l_0$};
			\node[good state] at (-2,-2)  (S1) {$l_1$};
			\node[bad state] at (4,-2)  (S2)  {$\begin{array}{c}\bm{l_2}\\ c<a\end{array}$};
			\node[dead state] at (0.5,-4) (S3)  {$l_3$};

            \path (S0) edge node [el,above] {$\varphi/\mu(x)$}( S1)
            edge node [el,above] {$\neg \varphi, c:=0 /\mu(x)$} (S2)    
			(S1) edge [loop left] node [el,above] {$\varphi/\mu(x)$} (S1)  
            edge [bend right] node {$\neg \varphi, c:=0/ \mu(x)$} (S2)   
			(S2) edge [loop below] node {$\neg \varphi, c < a/\mu(x)$} (S2)
            edge node {$\varphi, c \leq a/\mu(x)$} (S1)  
            edge [loop above]  node {$\neg \varphi, c== a; c:=0/ \mu(x)=0.7$} (S2)  
            edge node [el,below] {$\top, c>a/ vio$} (S3)
            (S3) edge [loop left] node {$\top/ vio$} (S3);
		\end{tikzpicture}
  \caption{}
  \end{figure}

    \begin{proposition} Proposition (Equivalence of TA and STL.)
    \end{proposition} 

==> sections/operators/release.tex <==
\subsubsection{Timed Transducer for $\varphi_1\release_{[a,b]}\varphi_2$}       
        We let $\automaton=(\loca,\linit,\clock,\allowbreak\alphbt,\trans, \lambda, \lacpt)$, where
        \begin{itemize}
            \item $\loca=\{l_0, l_1, l_2, l_3\}$ 
            
            \item $\linit=l_0$ 
            
            \item $\clock=\{c\}$
            
            \item $\allowbreak\alphbt=\{\varphi_1, \neg \varphi_1, \varphi_2, \neg \varphi_2\}$
            
            \item $\trans=\{ \delta_1 \cdots \delta_{15} \}$
            
            %\item \sout{$Inv(l_2): c<b$} \\
            %$Inv=\{(l_0,\emptyset),(l_1,c<b),(l_2,\emptyset), (l_3,c<b), (l_4, \emptyset) \}$

            
            \item $\lambda=\{\lambda_1 \cdots \lambda_{15}\}$
            \item $\lacpt=\{l_2\}$
        \end{itemize}

        \begin{table}[H]
        \scalebox{0.9}{
        \begin{tabular}{@{}ccc@{}}
        \hline
        i & $\delta_i$                   & $\lambda_i$ \\ \hline
        1 & $(l_0, \neg \varphi_1, \epsilon, c:=0, l_1)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$ \\ 
        2 & $(l_0, \varphi_1, \epsilon, \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\ 

        3 & $(l_1, \neg \varphi_1, c<a, \epsilon, l_1)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\ 
        
        4 & $(l_1,  \varphi_1 , c <a , \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$ \\ 
        5 & $(l_1, \varphi_1 \land \varphi_2, c =a , \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$   \\
        6 & $(l_1, \varphi_1 \land \neg \varphi_2, c =a , \epsilon, l_2)$ & $\varphi_2(\mu(\signal_i), \cdots, \mu(\signal_k))=true$ \\
        
        7 & $(l_1, \neg \varphi_1 \land \neg \varphi_2 , c =a , \epsilon, l_3)$ & $\varphi_2(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\
        8 & $(l_1, \neg \varphi_1 \land \varphi_2, c =a , \epsilon, l_3)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\

        9 & $(l_2, \Sigma, \epsilon , \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\
        
        10 & $(l_3, \neg \varphi_1 \land \neg \varphi_2, c \geq a \text{ and } c < b , \epsilon, l_3)$ & $\varphi_2(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\
        11 & $(l_3, \neg \varphi_1 \land \varphi_2, c \geq a \text{ and } c < b , \epsilon, l_3)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\
        
        12 & $(l_3, \varphi_1 \land \varphi_2,  c \geq a \text{ and } c \leq b, \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$ \\
        13 & $(l_3, \varphi_1 \land \neg \varphi_2,  c \geq a \text{ and } c \leq b, \epsilon, l_2)$ & $\varphi_2(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\
        14 & $(l_3,  \neg \varphi_1 \land  \neg \varphi_2,  c =b, \epsilon, l_2)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true $  \\
        & & $~\land \varphi_2(\mu(\signal_i), \cdots, \mu(\signal_k))=true$\\
        15 & $(l_3, \neg \varphi_1 \land \varphi_2,  c=b, \epsilon, l_2)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\
        % 17 & $(l_3, \neg \varphi_1 \land \neg \varphi_2,  c = b, \epsilon, l_2)$ & $\mu(x_1)=0.7\land \mu(x_2)=0.9$  \\
        % 18 & $(l_3, \neg \varphi_1 \land \varphi_2,  c =b, \epsilon, l_2)$ & $\mu(x_1) =0.7 \land \mu(x_2) $  \\
        
        % 19 & $(l_4, \Sigma, \epsilon, \epsilon, l_4)$ & $vio$  \\
        
        \bottomrule
        \end{tabular}}
        \caption
        {Edges of Timed Transducer for $\varphi_1\release_{[a,b]}\varphi_2$ and their output labels.}
        \label{table:release}
        \end{table}




% \hscomment{yes, I think it's right! But I have some other question: is the blue transition necessary?}
% \saucomment{yes blue transitions are requiered}
\begin{figure}[H]
        \centering
        \begin{tikzpicture}[->,shorten >=1pt,auto,node distance=3.5cm,el/.style = {inner sep=2pt, align=left, sloped},every label/.append style = {font=\small},semithick,initial where=above]
			
			\tikzstyle{every node}=[font=\small]
			\tikzstyle{good state}=[circle,thick,draw=blue!75,fill=blue!20,minimum size=5mm,accepting]
			\tikzstyle{bad state}=[circle,thick,draw=red!75,fill=red!20,minimum size=3mm]
			\tikzstyle{dead state}=[rectangle,thick,draw=red!75,fill=red!20,minimum size=5mm]

            \node[initial, bad state]  at (0,0) (S0) {$l_0$};
            \node[bad state] at (0,-2) (S1) {$l_1$};
            \node[good state] at (-2.5,-5.5) (S2) {$l_2$};
			\node[bad state] at (2.5,-5.5)  (S3) {$l_3$};
			%\node[dead state] at (0,-5)  (S4)  {$l_4$};
			
	%{$\begin{array}{c}\varphi_1, c<a /\top\\ \neg \varphi_1, c<a / \bot_1 \end{array}$}		
 %[bend right=70]
			\path (S0) edge node {$\neg \varphi_1, x:=0 / \top$}(S1)
            edge [bend right=40] node [el,above] {$ \varphi_1 / \top$}(S2)
            
            (S1) edge [loop right] node {$\neg \varphi_1, c<a / \top$} (S1)
            edge node [el,above] {$\begin{array}{c}\neg \varphi_1 \land \neg \varphi_2, c =a/ \bot_2\\ \neg \varphi_1 \land \varphi_2, c =a/ \top \end{array}$} (S3)
            %edge node [el,below] {$\Sigma, c>b / vio$} (S4)
            
            edge node [el,above] {$\begin{array}{c} 
            \varphi_1, c < a / \top\\
            \varphi_1 \land \varphi_2, c =a/ \top\\
            %%
            % \blue{\neg \varphi_1 \land \neg \varphi_2, c=b/ \bot_1, \bot_2}\\
            % \blue{\neg \varphi_1 \land \varphi_2, c =b/ \bot_1}\\
            %%
            \varphi_1 \land \neg \varphi_2, c =a/ \bot_2\\ \end{array}$} (S2)
            
            (S2) edge [loop below] node {$\Sigma / \top$} (S2)
            
            (S3) edge [loop right] node [el,above]  {$\begin{array}{c}\neg \varphi_1 \land \neg \varphi_2, c \geq a \text{ and } c<b / \bot_2\\
            \neg \varphi_1 \land \varphi_2, c \geq a \text{ and } c<b / \top\end{array}$} (S3)
            %
            %edge node [el,below] {$\Sigma, c>b / vio$} (S4)
            %
            edge node {$\begin{array}{c}\varphi_1 \land  \varphi_2, c \geq a \text{ and } c \leq b/ \top\\
            \varphi_1 \land \neg \varphi_2, c \geq a \text{ and } c \leq b/ \bot_2\\
            %%
            \neg \varphi_1 \land \neg \varphi_2, c =b/ \bot_1, \bot_2\\
            \neg \varphi_1 \land \varphi_2, c =b/ \bot_1 \end{array}$} (S2);
            
            %(S4) edge [loop below] node {$\Sigma / vio$} (S4);
		\end{tikzpicture}
  \caption{Timed Transducer for $\varphi_1\release_{[a,b]}\varphi_2$}
  \label{fig: release}
  \end{figure}




  


==> sections/operators/until.tex <==
\subsubsection{Timed Transducer for $\varphi_1\until_{[a,b]}\varphi_2$}       
        We let $\automaton=(\loca,\linit,\clock,\allowbreak\alphbt,\trans, \lambda, \lacpt)$, where
        \begin{itemize}
            \item $\loca=\{l_0, l_1, l_2, l_3\}$ %\sout{where $observing=\{l_0, l_1, l_2, l_3\}$, $modifying=\{l4\}$ and $violation=\{l5\}$}
            
            \item $\linit=l_0$ 
            
            \item $\clock=\{c\}$
            
            \item $\allowbreak\alphbt= \{\varphi_1, \neg \varphi_1, \varphi_2, \neg \varphi_2\}$
            
            \item %$\trans=\{ \delta_1, \delta_2, \delta_3,\delta_4, \delta_5, \delta_6, \delta_7, \delta_8,\delta_9, \delta_{10},\delta_{11},\delta_{12} \}$
            $\trans=\{ \delta_1, \cdots ,\delta_{15} \}$
            
            %\item %\sout{$Inv(l_2): c<b$} \\
            %$Inv=\{(l_0,\emptyset),(l_1,\emptyset),(l_2,\emptyset), (l_3,\emptyset), (l_4, c<b), (l_4,\emptyset)\}$

            
            \item %$\lambda=\{\lambda_1, \lambda_2, \lambda_3, \lambda_4, \lambda_5, \lambda_6, \lambda_7, \lambda_8, \lambda_9, \lambda_{10}, \lambda_{11}, \lambda_{12}\}$
            $\lambda=\{\lambda_1,\cdots \lambda_{15}\}$
            \item $\lacpt=\{l_2\}$
        \end{itemize}
\begin{remark}
    The output labels $\lambda_i$ corresponding to the transition $\delta_i$ in Tables \ref{table:until} and \ref{table:release} represent the value of the signal outputted by the timed transducer such that the predicates are satisfied. For signals $(\signal_1, \cdots, \signal_k)$, and predicates $(\varphi_1, \cdots, \varphi_n)$, $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$ represents that the value of all the signals is not modified by the timed transducer, however, $\varphi_p(\mu(\signal_i), \cdots, \mu(\signal_k))=true$ represents that the value of (some or all) the signals is (minimally) modified by the timed transducer to satisfy the proposition $p$.

    To simplify and clean up the Figures \ref{fig: until} and \ref{fig: release}, we denote $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$ by simply $\top$ (meaning no change in signals value) and $\varphi_p(\mu(\signal_i), \cdots, \mu(\signal_k))=true$ by $\bot_p$ (meaning signals value changed to satisfy proposition $p$).
    
\end{remark}
    
        \begin{table}[H]
        \scalebox{0.9}{
        \begin{tabular}{@{}ccc@{}}
        \hline
        i & $\delta_i$                   & $\lambda_i$ \\ \hline
        1 & $(l_0, \varphi_1, \epsilon, c:=0, l_1)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\ 
        2 & $(l_0, \neg \varphi_1, \epsilon, c:=0, l_1)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true$ \\ 
        
        % 3 & $(l_1, \neg \varphi_1, c<a, \epsilon, l_2)$ & $\mu(x_1)=0.7 \land \mu(x_2)$  \\ 
        % 4 & $(l_1, \Sigma, c>b, \epsilon, l_5)$ & $vio$  \\ 
        
        3 & $(l_1, \varphi, c<a, \epsilon, l_1)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\ 
        4 & $(l_1, \neg \varphi, c <a, \epsilon, l_1)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\ 
        
        5 & $(l_1, \varphi \land \varphi_2, c=a, \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\ 
        6 & $(l_1, \neg \varphi_1 \land \varphi_2, c=a, \epsilon, l_2)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\
        
        % 7 & $(l_1, \varphi_1 \land \varphi_2, c \geq a \text{ and } c \leq b , \epsilon, l_1)$ & $\mu(x_1) \land \mu(x_2)$  \\ 
        % 8 & $(l_1, \varphi_1 \land \neg \varphi_2, c=b, \epsilon, l_1)$ & $\mu(x_1) \land \mu(x_2)$  \\ 
        7 & $(l_1, \varphi_1 \land \neg \varphi_2, c =a, \epsilon, l_3)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$ \\
        8 & $(l_1, \neg \varphi_1 \land \neg \varphi_2, c=a, \epsilon, l_3)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true$ \\
        
        9 & $(l_2, \Sigma, \epsilon, \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\ 

        10 & $(l_3, \varphi \land \neg \varphi_2, c \geq a \text{ and } c<b , \epsilon, l_3)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\ 
        11 & $(l_3, \neg \varphi \land \neg \varphi_2, c \geq a \text{ and } c<b, \epsilon, l_3)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\ 
        
        12 & $(l_3, \varphi_1 \land \varphi_2, c \geq a \text{ and } c \leq b, \epsilon, l_2)$ & $\mu(\signal_s)'=\mu(\signal_s), \forall s= 1, \cdots, k$  \\
        13 & $(l_3, \neg \varphi_1 \land \varphi_2, c \geq a \text{ and } c \leq b, \epsilon, l_2)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\
        14 & $(l_3, \neg \varphi_1 \land \neg \varphi_2, c =b, \epsilon, l_2)$ & $\varphi_1(\mu(\signal_i), \cdots, \mu(\signal_k))=true $  \\
        & &$\land ~\varphi_2(\mu(\signal_i), \cdots, \mu(\signal_k))=true$\\
        15 & $(l_3, \varphi_1 \land \neg \varphi_2, c =b, \epsilon, l_2)$ & $\varphi_2(\mu(\signal_i), \cdots, \mu(\signal_k))=true$  \\
        
        % 16 & $(l_3, \Sigma, c>b, \epsilon, l_4)$ & $vio$  \\
        % 17 & $(l_4, \Sigma, \epsilon, \epsilon, l_4)$ & $vio$  \\
        \bottomrule
        \end{tabular}}
        \caption
        {Edges of Timed Transducer for $\varphi_1\until_{[a,b]}\varphi_2$ and their output labels.}
        \label{table:until}
        \end{table}





% \hscomment{I believe the label $\neg \varphi_1\land\varphi_2, c=b / \bot_1$ in transition from $l_3$ to $l_2$ should be modified into $\neg\varphi_1\land \varphi_2, a\le c\le b / \bot_1$. Let's discuss tomorrow!}
% \saucomment{yes, u r right, I modified it}
  \begin{figure}[H]
        \centering
        \begin{tikzpicture}[->,shorten >=1pt,auto,node distance=3.5cm,el/.style = {inner sep=2pt, align=left, sloped},every label/.append style = {font=\small},semithick,initial where=above]
			
			\tikzstyle{every node}=[font=\small]
			\tikzstyle{good state}=[circle,thick,draw=blue!75,fill=blue!20,minimum size=5mm,accepting]
			\tikzstyle{bad state}=[circle,thick,draw=red!75,fill=red!20,minimum size=3mm]
			\tikzstyle{dead state}=[rectangle,thick,draw=red!75,fill=red!20,minimum size=5mm]

            \node[initial, bad state]  at (0,0) (S0) {$l_0$};
            %\node[bad state] at (0,-1) (S1) {$l_1$};
            \node[bad state] at (0,-2) (S2) {$l_1$};
			\node[good state] at (-2.5,-5)  (S3) {$l_2$};
			\node[bad state] at (2.5,-5)  (S4)  {$l_3$};
			%\node[dead state] at (0,-5) (S5)  {$l4$};
			
0			\path (S0) edge node {$\begin{array}{c}\varphi_1, c:=0, / \top\\ \neg \varphi_1, c:=0, / \bot_1  \end{array}$}(S2)
            % (S1) edge node {$\begin{array}{c}\varphi_1, c<a /\top\\ \neg \varphi_1, c<a / \bot_1 \end{array}$} (S2)
            % edge [bend right=20] node [el,below] {$\Sigma, c>b/vio$} (S5)
            %%edge [bend right=70] node [el,below] {$\Sigma, c \geq a, c \leq b/vio$} (S5)
            
            (S2) edge [loop right] node  {$\begin{array}{c} \varphi_1, c<a / \top \\
            \neg \varphi_1, c<a/ \bot_1 \end{array}$} (S2)
            edge node [el,above] {$\begin{array}{c}\varphi_1 \land \varphi_2, c =a / \top\\
            \neg \varphi_1 \land \varphi_2, c =a / \bot_1\end{array}$} (S3)
            edge node [el,above] {$\begin{array}{c}\varphi_1 \land \neg \varphi_2, c=a / \top\\
            \neg \varphi_1 \land \neg \varphi_2, c=a / \bot_1
            \end{array}$} (S4)
            %edge node [el,above] {$\Sigma, c>b/vio$} (S5)

			(S3) edge [loop below] node {$\Sigma/ \top$} (S3)
            
            (S4) edge [loop right] node [el,above] {$\begin{array}{c}\varphi_1 \land \neg \varphi_2, c \geq a, c < b / \top\\ 
            \neg \varphi_1 \land \neg \varphi_2, c \geq a, c < b/ \bot_1  \end{array}$} (S4)
            edge node {$\begin{array}{c} \varphi_1 \land  \varphi_2, a \leq c \leq b / \top\\
            \neg \varphi_1 \land  \varphi_2, a \leq c \leq b / \bot_1\\
             \varphi_1 \land \neg \varphi_2, c = b / \bot_2\\
             \neg \varphi_1 \land \neg \varphi_2, c=b / \bot_1, \bot_2\end{array} $} (S3);
            %edge  node [el,above] {$\Sigma, c>b/vio$} (S5)
            
            %(S5) edge [loop below] node {$\Sigma/ vio$} (S5);
		\end{tikzpicture}
  \caption{Timed Transducer for $\varphi_1\until_{[a,b]}\varphi_2$}
  \label{fig: until}
  \end{figure}
    




    

  
  %   \begin{figure}[H]
  %       \centering
  %       \begin{tikzpicture}[->,shorten >=1pt,auto,node distance=3.5cm,el/.style = {inner sep=2pt, align=left, sloped},every label/.append style = {font=\small},semithick,initial where=above]
			
		% 	\tikzstyle{every node}=[font=\small]
		% 	\tikzstyle{good state}=[circle,thick,draw=blue!75,fill=blue!20,minimum size=5mm,accepting]
		% 	\tikzstyle{bad state}=[circle,thick,draw=red!75,fill=red!20,minimum size=3mm]
		% 	\tikzstyle{dead state}=[rectangle,thick,draw=red!75,fill=red!20,minimum size=5mm]

  %           \node[initial, good state]  at (0,1.5) (S4) {$l_1$};
  %           \node[bad state] (S0) {$l_0$};
		% 	\node[good state] at (-2.5,-5)  (S1) {$l_2$};
		% 	\node[bad state] at (2.5,-5)  (S2)  {$\begin{array}{c}\bm{l_3}\\ c<a\end{array}$};
		% 	\node[dead state] at (0,-6.5) (S3)  {$l4$};
			
		% 	\path (S0) edge node [el,above] {$\varphi_1 \land \varphi_2, c>a/ \mu(x_1) \land \mu(x_2)$}(S1)
  %           edge node [el,above] {$\varphi_1 \land \neg \varphi_2,c>a, c:=0/ \mu(x_1) \land \mu(x_2)$} (S2)  edge [loop right] node {$\top, c<a / \mu(x_1) \land \mu(x_2) $} (S3)    
            
  %           edge  node [el,above] {$\neg \varphi_1 / vio $} (S3)    
		% 	(S1) edge [loop left] node [el,above] {$\varphi_1 \land  \varphi_2/ \mu(x_1) \land \mu(x_2)$} (S1)
  %           edge node {$\varphi_1 \land \neg \varphi_2, c:=0/ \mu(x_1) \land \mu(x_2)$} (S2)
  %           edge [bend right] node [el,below] {$\neg \varphi_1 / vio$} (S3)   
		% 	(S2) edge [loop right] node [el,above] {$\begin{array}{c}\varphi_1 \land  \neg \varphi_2, c < a /\mu(x_1) \land \mu(x_2) \\ p_1 \land  \neg \varphi_2, c==a / \mu(x_1)=0.7 \land \mu(x_2)=0.7 \end{array}$} (S2)
  %           edge [bend left] node [el,above]{$\varphi_1 \land \varphi_2, c\leq a/ \mu(x_1) \land \mu(x_2)$} (S1) 
  %           edge [bend left] node [el,below] {$\begin{array}{c} \top, c>a/ vio\\ ~\neg \varphi_1/ vio\end{array}$} (S3)
  %           (S3) edge [loop below] node {$\top/ vio$} (S3)
            
  %           (S4) edge node {$\top, c:=0/ \mu(x_1) \land \mu(x_2)$} (S0);
		% \end{tikzpicture}
  % \end{figure}



==> sections/sec_results.tex <==
\section{Main Results}
\label{sec:results}
We now state the soundness and completeness of the translation of the STL formulas into the transducers.

We propose here the equivalence of the Until and Release operator of STL and its transducer. %A similar proof is done for the Release operator of STL and its transducer.

\hscomment{1. Include the output alphabet $\top, \bot$, not the input (thius can be used to prove the transparancy), 2. CHange the notation. 3. Move it to Section 4.}
\begin{proposition}[Equivalence of Until operator of STL and its transducer]    
\label{propo1}
        Let $\signal$ be the signals and $\textsf{SignEncode}(\signal,\varphi_1\until_{[a,b]}\varphi_2)$ be its encoded timed word for the given STL formula $\varphi_1\until_{[a,b]}\varphi_2$.
        If the encoded timed word is accepted by the transducer of Until operator $\automaton_{\varphi_1\until_{[a,b]}\varphi_2}$ then the corresponding signals  $\signal$  satisfy $ \varphi_1\until_{[a,b]}\varphi_2$, i.e.,
        \begin{align*}
            \textsf{SignEncode}(\signal,\varphi_1\until_{[a,b]}\varphi_2) \in \mathcal{L}(\automaton_{\varphi_1\until_{[a,b]}\varphi_2}) \implies \signal \models \varphi_1\until_{[a,b]}\varphi_2
        \end{align*}
\end{proposition}

\begin{proposition}[Equivalence of Release operator of STL and its transducer]   
\label{propo2}
    %Let $\signal$ be the signals.
    %Let $\sigma$ be the timed word. 
    Let $\signal$ be the signals and $\textsf{SignEncode}(\signal,\varphi_1\release_{[a,b]}\varphi_2)$ be its encoded timed word for the given STL formula $\varphi_1\release_{[a,b]}\varphi_2$
    If the timed word is accepted by the transducer of Release operator $\automaton_{\varphi_1\release_{[a,b]}\varphi_2}$ then the corresponding  signals $\signal$ satisfy $ \varphi_1\release_{[a,b]}\varphi_2$, i.e.,
    \begin{align*}
        \textsf{SignEncode}(\signal,\varphi_1\release_{[a,b]}\varphi_2) \in \mathcal{L}(\automaton_{\varphi_1\release_{[a,b]}\varphi_2}) \implies \signal \models \varphi_1\release_{[a,b]}\varphi_2
    \end{align*}
\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{proposition} 
\label{propo3}
    Let $\signal$ be the signals and let $\textsf{SignEncode}(\signal,\varphi_1\until_{[a,b]}\varphi_2)$ be the corresponding encoded timed word. If signals  satisfy the Until formula $ \varphi_1\until_{[a,b]}\varphi_2$, then its encoded word is accepted by its transducer, i.e., 
    \begin{align*}
        \signal \models \varphi_1\until_{[a,b]}\varphi_2 \implies \textsf{SignEncode}(\signal,\varphi_1\until_{[a,b]}\varphi_2) \in 
        \mathcal{L}(\automaton_{\varphi_1\until_{[a,b]}\varphi_2}) 
    \end{align*}
\end{proposition}

\begin{proposition} 
\label{propo4}
    Let $\signal$ be the signals and let $\textsf{SignEncode}(\signal,\varphi_1\release_{[a,b]}\varphi_2)$ be the corresponding encoded timed word. If signals  satisfy the Release formula $ \varphi_1\release_{[a,b]}\varphi_2$, then its encoded word is accepted by its transducer, i.e., 
    \begin{align*}
        \signal \models \varphi_1\release_{[a,b]}\varphi_2 \implies \textsf{SignEncode}(\signal,\varphi_1\release_{[a,b]}\varphi_2) \in 
        \mathcal{L}(\automaton_{\varphi_1\release_{[a,b]}\varphi_2}) 
    \end{align*}
\end{proposition}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{proposition} 
% \label{propo5}
%     Let $\signal$ be the signals and let $\sigma$ be the corresponding encoded timed word. If signals do not satisfy the Until formula $ \varphi_1\until_{[a,b]}\varphi_2$, and the enforcer corrects the signals to $\signal'$ by minimally modifying $\signal$ and the encoded signals of the modified signals are accepted by the transducer of Until, then the modified signals satisfy  the Until formula, i.e., 
%     \begin{equation*}    
%         \begin{split}
%         \signal \not \models p_1\until_{[a,b]}p_2 \land \exists\signal', E_{p_1\until_{[a,b]}p_2}(\signal, t)=\signal' : min(|\signal'-\signal|)\\ \land \sigma' \in 
%         \mathcal{L}(\automaton_{\varphi_1\release_{[a,b]}\varphi_2}) 
%         \implies \signal' \models p_1\until_{[a,b]}p_2
%         \end{split}
%     \end{equation*}    
% \end{proposition}

% \begin{proposition} 
% \label{propo6}
%     Let $\signal$ be the signals and let $\sigma$ be the corresponding encoded timed word. If signals do not satisfy the Until formula $ \varphi_1\release_{[a,b]}\varphi_2$, and the enforcer corrects the signals to $\signal'$ by minimally modifying $\signal$ and the encoded signals of the modified signals are accepted by the transducer of Release, then the modified signals satisfy  the Release formula, i.e.,
%     \begin{equation*}    
%         \begin{split}
%         \signal \not \models p_1\release_{[a,b]}p_2 \land \exists\signal', E_{p_1\release_{[a,b]}p_2}(\signal, t)=\signal' : min(|\signal'-\signal|)\\ \land \sigma' \in 
%         \mathcal{L}(\automaton_{\varphi_1\release_{[a,b]}\varphi_2}) 
%         \implies \signal' \models p_1\release_{[a,b]}p_2
%         \end{split}
%     \end{equation*}    
% \end{proposition}


The proofs of the propositions are provided at Appendix \ref{sec:appendix}.

==> sections/sec_results1.tex <==
\section{Main Results}
\label{sec:results}
We now state the soundness and completeness of the translation of the STL formulas into the transducers.

We propose here the equivalence of the Until and Release operator of STL and its transducer. %A similar proof is done for the Release operator of STL and its transducer.
%\hscomment{The notation we use should be align with that in \cref{sec: Transform STL into TA}. $\varphi_1\until_I\varphi_2$ should be $p_1\until p_2$.}

\begin{proposition}[Equivalence of Until operator of STL and its transducer]    
\label{propo1}
        Let $\signal$ be the signals. Let $\tword$ be its encoded timed word for the given STL formula $p_1\until_{[t_1,t_2]}p_2$. %Let $\rho$ be the run of $\automaton_{p_1\until_{[t_1,t_2]}p_2}$ over $\sigma$ from its initial state. 
        Let $\bm{\omega}_{\top}$ be the output timed word for the accepting run over $\tword$, where the output of all transition being $\top$. Then,

        
        %If the encoded timed word is accepted by the transducer of Until operator $\automaton_{p_1\until_{[t_1,t_2]}p_2}$, and the output of  all the transitions for that accepting run,  is $\top$ then the corresponding signals  $\signal$  satisfy $ p_1\until_{[t_1,t_2]}p_2$, i.e.,
        %\hscomment{We have not define the notion $\mathcal{L}(\automaton)$. Please refer to \cref{sec:Preliminaries and notations} for the notation of $\bm{\omega} = \llangle\automaton\rrangle(\tword)$ in line 240-244, I defined this notation specifically for writing the proposition.}
        % \begin{align*}
        %     %\sigma \in \mathcal{L}(\automaton_{p_1\until_{[t_1,t_2]}p_2})  \land \forall \delta \in \rho, \lambda(\delta)=\top \implies \signal \models p_1\until_{[t_1,t_2]}p_2
        %     \llangle\automaton_{p_1\until_{[t_1,t_2]}p_2}\rrangle(\tword) \land \forall \delta \in \rho, \lambda(\delta)=\top \implies \signal \models p_1\until_{[t_1,t_2]}p_2
        % \end{align*}
        % \hscomment{Is this version more clear?}
        % \saucomment{yes. only thing is that: we cant use $SignEncode$ because SignEncode gives timed event at time t and not the entire encoded-word for the $\signal$}
        % \hscomment{okay, this version is more suitable.}
        %Let \(\signal\) be the signal and \(\tword = \textsf{SignEncode}(p_1 \until_I p_2, \signal)\). Let $\bm{\omega}_{\top}$ denote the timed word where the action of all its events is $\top$. Then,
        \[
            \llangle\automaton_{\until}\rrangle(\tword) = \bm{\omega}_{\top} \iff \signal \models p_1 \until_{[t_1, t_2]} p_2
        \]
        
\end{proposition}

\begin{proposition}[Equivalence of Release operator of STL and its transducer]   
\label{propo2}
    Let $\signal$ be the signals. Let $\tword$ be its encoded timed word for the given STL formula $p_1\release_{[t_1,t_2]}p_2$. %Let $\rho$ be the run of $\automaton_{p_1\release_{[t_1,t_2]}p_2}$ over $\sigma$ from its initial state. 
    Let $\bm{\omega}_{\top}$ be the output timed word for the accepting run over $\tword$, where the output of all transitions being $\top$. Then,
        
        %If the encoded timed word is accepted by the transducer of Until operator $\automaton_{p_1\release_{[t_1,t_2]}p_2}$, and the output of  all the transitions for that accepting run,  is $\top$ then the corresponding signals  $\signal$  satisfy $ p_1\release_{[t_1,t_2]}p_2$, i.e.,

        \begin{align*}
        \llangle\automaton_{\release}\rrangle(\tword) = \bm{\omega}_{\top} \implies \signal \models p_1 \release_{[t_1, t_2]} p_2
        %\sigma \in \mathcal{L}(\automaton_{p_1\release_{[t_1,t_2]}p_2})  \land \forall \delta \in \rho, \lambda(\delta)=\top \implies \signal \models p_1\until_{[t_1,t_2]}p_2
        \end{align*}
\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{proposition} 
% \label{propo3}
%     Let $\signal$ be the signals and let $\tword$ be the corresponding encoded timed word. If signals  satisfy the Until formula $ p_1\until_{[t_1,t_2]}p_2$, then its encoded word is accepted by its transducer, i.e., 
%     \begin{align*}
%         \signal \models p_1\until_{[t_1,t_2]}p_2 \implies \llangle\automaton_{\until}\rrangle(\tword) \red{=\bm{\omega}_{\top}} %\sigma \in \mathcal{L}(\automaton_{p_1\until_{[t_1,t_2]}p_2}) 
%     \end{align*}
% \end{proposition}

% \begin{proposition} 
% \label{propo4}
%     Let $\signal$ be the signals and let $\tword$ be the corresponding encoded timed word. If signals  satisfy the Release formula $ p_1\release_{[t_1,t_2]}p_2$, then its encoded word is accepted by its transducer, i.e., 
%     \begin{align*}
%         \signal \models p_1\release_{[t_1,t_2]}p_2 \implies \llangle\automaton_{\until}\rrangle(\tword) %\tword \in \mathcal{L}(\automaton_{p_1\release_{[t_1,t_2]}p_2}) 
%     \end{align*}
% \end{proposition}

The proofs of the propositions are provided in Appendix \ref{sec:appendix}.

==> tikz.tex <==
\RequirePackage{tikz}
\RequirePackage{pgfplots}

\usetikzlibrary{
	cd,
	math,
	decorations.markings,
	decorations.pathreplacing,
	positioning,
	arrows.meta,
	circuits.logic.US,
	shapes,
	calc,
	fit,
	quotes,
  scopes,
  patterns,
  backgrounds}

\usepgfplotslibrary{groupplots, fillbetween}
\usetikzlibrary{calc, positioning, arrows.meta }
\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark}
\usetikzlibrary{arrows,shapes,positioning,shadows,trees,mindmap}

\tikzset{
        oriented WD/.style={%everything after equals replaces "oriented WD" in key.
           %every to/.style={out=0,in=180,draw},
           label/.style={
              font=\everymath\expandafter{\the\everymath\scriptstyle},
              inner sep=0pt,
              node distance=2pt and -2pt},
           semithick,
           node distance=1 and 1,
           decoration={markings, mark=at position \stringdecpos with \stringdec},
           ar/.style={postaction={decorate}},
           execute at begin picture={\tikzset{
              x=\bbx, y=\bby,
              every fit/.style={inner xsep=\bbx, inner ysep=\bby}}}
           },
        string decoration/.store in=\stringdec,
        string decoration={\arrow{stealth};},
        string decoration pos/.store in=\stringdecpos,
        string decoration pos=.7,
        bbx/.store in=\bbx,
        bbx = 1.5cm,
        bby/.store in=\bby,
        bby = 1.5ex,
        bb port sep/.store in=\bbportsep,
        bb port sep=1.5,
        % bb wire sep/.store in=\bbwiresep,
        % bb wire sep=1.75ex,
        bb port length/.store in=\bbportlen,
        bb port length=4pt,
        bb penetrate/.store in=\bbpenetrate,
        bb penetrate=0,
        bb min width/.store in=\bbminwidth,
        bb min width=1cm,
        bb rounded corners/.store in=\bbcorners,
        bb rounded corners=2pt,
        bb small/.style={bb port sep=1, bb port length=2.5pt, bbx=.4cm, bb min width=.4cm, 
   bby=.7ex},
            bb medium/.style={bb port sep=1, bb port length=2.5pt, bbx=.4cm, bb min width=.4cm, 
   bby=.9ex},
        bb/.code 2 args={%When you see this key, run the code below:
           \pgfmathsetlengthmacro{\bbheight}{\bbportsep * (max(#1,#2)+1) * \bby}
           \pgfkeysalso{draw,minimum height=\bbheight,minimum width=\bbminwidth,outer 
   sep=0pt,
              rounded corners=\bbcorners,thick,
              prefix after command={\pgfextra{\let\fixname\tikzlastnode}},
              append after command={\pgfextra{\draw
                 \ifnum #1=0{} \else foreach \i in {1,...,#1} {
%                    ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(-\bbportlen,0) coordinate (\fixname_in\i) -- +(\bbpenetrate,0) coordinate (\fixname_in\i')}\fi 
                    ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(0,0) coordinate (\fixname_in\i) -- +(\bbpenetrate,0) coordinate (\fixname_in\i')}\fi 
     %Define the endpoints of tickmarks
                 \ifnum #2=0{} \else foreach \i in {1,...,#2} {
%                    ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(-\bbpenetrate,0) coordinate (\fixname_out\i') -- +(\bbportlen,0) coordinate (\fixname_out\i)}\fi;
                    ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(-\bbpenetrate,0) coordinate (\fixname_out\i') -- +(0,0) coordinate (\fixname_out\i)}\fi;
              }}}
        },
        bb name/.style={append after command={\pgfextra{\node[anchor=north] at 
   (\fixname.north) {#1};}}}     
}

\tikzset{bubble/.style={%
  rectangle,
  thick,
  draw=#1,
  rounded corners,
  fill=#1!20,
  align=flush center,
  minimum height=0.8cm,
  minimum width=1.5cm
  }
}

\tikzset{
  sine wave icon/.style={
    circle,  
    draw=black,  
    fill=gray!10,
    minimum size=1.5cm,  
    path picture={  
      \draw[domain=-0.31415:0.31415, samples=50, smooth]
        plot (\x, {0.3*sin(10*\x r)});  
    }
  }
}
\newcommand{\highlight}[2]{\colorbox{#1!17}{$\displaystyle #2$}}
\newcommand{\highlightdark}[2]{\colorbox{#1!47}{$\displaystyle #2$}}
\renewcommand{\highlight}[2]{\colorbox{#1!17}{#2}}
\renewcommand{\highlightdark}[2]{\colorbox{#1!47}{#2}}
